Exploring Latent Pathways: Enhancing the Interpretability of Autonomous Driving with a Variational Autoencoder

Autonomous driving presents a complex challenge, which is usually addressed with artificial intelligence models that are end-to-end or modular in nature. Within the landscape of modular approaches, a bio-inspired neural circuit policy model has emerged as an innovative control module, offering a compact and inherently interpretable system to infer a steering wheel command from abstract visual features. Here, we take a leap forward by integrating a variational autoencoder with the neural circuit policy controller, forming a solution that directly generates steering commands from input camera images. By substituting the traditional convolutional neural network approach to feature extraction with a variational autoencoder, we enhance the system's interpretability, enabling a more transparent and understandable decision-making process. In addition to the architectural shift toward a variational autoencoder, this study introduces the automatic latent perturbation tool, a novel contribution designed to probe and elucidate the latent features within the variational autoencoder. The automatic latent perturbation tool automates the interpretability process, offering granular insights into how specific latent variables influence the overall model's behavior. Through a series of numerical experiments, we demonstrate the interpretative power of the variational autoencoder-neural circuit policy model and the utility of the automatic latent perturbation tool in making the inner workings of autonomous driving systems more transparent.

==> appendices/automatic_latent_plot.tex <==
The standard technique to interpret the information encoded in each latent dimension of VAE is to perform a latent perturbation analysis. This consists of taking the latent encoding of a given input, then to change the value of only one perturbation at the time and observe the change in the reconstructed image. For a small number of dimensions, the analysis can be carried out by an experienced human operator in a reasonable time. However in the  case of large number of dimensions, this operation becomes intractable for human. Additionally, a higher number of dimension means that the information is more diffused thus noticing the changes in the perturbated  reconstructions becomes highly difficult even for the eye of a trained expert, for example see \autoref{fig:dim0}

\begin{figure*}[!htb]
	\includegraphics[width=\textwidth]{material/dim0.png}
	\caption{Latent perturbation for latent dimension 0 (out of 256). The image in the center is the original input image. The images on the right and extreme-right represent respectively the perturbated reconstructions of the center image by adding respectively +1$\sigma$ and +$\sigma$ from the value of dimension 0. The images on the left and extreme-left represent respectively the perturbated reconstructions of the center image by subtracting respectively +1$\sigma$ and +$\sigma$ from the value of dimension 0. Here $\sigma$ represents the standard deviation of the distribution of the dimension 0.}
	\label{fig:dim0}
\end{figure*}

For this purpose, we developed an automatic assistant that indicates the detected changes and overlays them on top of the perturbated reconstruction. This simplifies the analysis task for the human operator and draws his attention to all possible differences between the extreme right and extreme left perturbated images as seen in \autoref{fig:alp0}.

\begin{figure}[!htb]
	\includegraphics[width=0.4\textwidth]{material/alp0.png}
	\caption{ALP plot for dimension 0. Top-center image represents the original input image. Top-right and top-left represent respectively the extreme-right and extreme-left images from \autoref{fig:dim0}. Bottom row images are each overlayed with the difference mask from \autoref{fig:diff0}, from left to right: extreme-left image, segmentation map of the (estimated using a DL model), extreme-right image.}
	\label{fig:alp0}
\end{figure}

\begin{figure}[!htb]
	\includegraphics[width=0.4\textwidth]{material/diff0.png}
	\caption{The difference image is obtained by subtracting the extreme-left image from the extreme-right one, then summing over the channels of its absolute value and finally thresholding over its normalization (by its maximum value) with the $90\textsuperscript{th}$ quantile as threshold.}
	\label{fig:diff0}
\end{figure}

==> appendices/usecases.tex <==
\begin{figure}[!htb]
	\includegraphics[width=0.4\textwidth]{material/usecase1.jpg}
	\label{fig:usecase1}
\end{figure}

\begin{figure}[!htb]
	\includegraphics[width=0.4\textwidth]{material/usecase2.jpg}
	\label{fig:usecase2}
\end{figure}

\begin{figure}[!htb]
	\includegraphics[width=0.4\textwidth]{material/usecase3.jpg}
	\label{fig:usecase3}
\end{figure}

\begin{figure}[!htb]
	\includegraphics[width=0.4\textwidth]{material/usecase4.jpg}
	\label{fig:usecase4}
\end{figure}

==> appendices/vae_archi.tex <==
\begin{figure*}[h]
	\begin{verbatim}
Model: "encoder"
__________________________________________________________________________________________________
Layer (type)                   Output Shape         Param #     Connected to                     
==================================================================================================
input_layer (InputLayer)       [(None, 78, 200, 4)  0           []                               
							   ]                                                                 

conv_1 (Conv2D)                (None, 39, 100, 8)   296         ['input_layer[0][0]']            

bn_1 (BatchNormalization)      (None, 39, 100, 8)   32          ['conv_1[0][0]']                 

relu_1 (ReLU)                  (None, 39, 100, 8)   0           ['bn_1[0][0]']                   

conv_2 (Conv2D)                (None, 20, 50, 16)   1168        ['relu_1[0][0]']                 

bn_2 (BatchNormalization)      (None, 20, 50, 16)   64          ['conv_2[0][0]']                 

relu_2 (ReLU)                  (None, 20, 50, 16)   0           ['bn_2[0][0]']                   

conv_3 (Conv2D)                (None, 10, 25, 32)   4640        ['relu_2[0][0]']                 

bn_3 (BatchNormalization)      (None, 10, 25, 32)   128         ['conv_3[0][0]']                 

relu_3 (ReLU)                  (None, 10, 25, 32)   0           ['bn_3[0][0]']                   

conv_4 (Conv2D)                (None, 5, 13, 64)    18496       ['relu_3[0][0]']                 

bn_4 (BatchNormalization)      (None, 5, 13, 64)    256         ['conv_4[0][0]']                 

relu_4 (ReLU)                  (None, 5, 13, 64)    0           ['bn_4[0][0]']                   

flatten (Flatten)              (None, 4160)         0           ['relu_4[0][0]']                 

mean (Dense)                   (None, 32)           133152      ['flatten[0][0]']                

log_var (Dense)                (None, 32)           133152      ['flatten[0][0]']                

sampling (Sampling)            (None, 32)           0           ['mean[0][0]',                   
'log_var[0][0]']                

==================================================================================================
Total params: 291,384
Trainable params: 291,144
Non-trainable params: 240
	\end{verbatim}
	\caption{Convolutional \acrshort{vae} encoder architecture.}
	\label{fig:encoder}
\end{figure*}

\begin{figure*}[h!]
	\begin{verbatim}
Model: "Decoder"
_________________________________________________________________
Layer (type)                Output Shape              Param #   
=================================================================
input_layer (InputLayer)    [(None, 32)]              0         

dense_1 (Dense)             (None, 4160)              137280    

Reshape (Reshape)           (None, 5, 13, 64)         0         

conv_transpose_1 (Conv2DTra  (None, 10, 26, 64)       36928     
nspose)                                                         

bn_1 (BatchNormalization)   (None, 10, 26, 64)        256       

relu_1 (ReLU)               (None, 10, 26, 64)        0         

conv_transpose_2 (Conv2DTra  (None, 20, 52, 32)       18464     
nspose)                                                         

bn_2 (BatchNormalization)   (None, 20, 52, 32)        128       

relu_2 (ReLU)               (None, 20, 52, 32)        0         

conv_transpose_3 (Conv2DTra  (None, 40, 104, 16)      4624      
nspose)                                                         

bn_3 (BatchNormalization)   (None, 40, 104, 16)       64        

relu_3 (ReLU)               (None, 40, 104, 16)       0         

conv_transpose_4 (Conv2DTra  (None, 80, 208, 8)       1160      
nspose)                                                         

bn_4 (BatchNormalization)   (None, 80, 208, 8)        32        

relu_4 (ReLU)               (None, 80, 208, 8)        0         

conv_transpose_5 (Conv2DTra  (None, 80, 208, 4)       292       
nspose)                                                         

resizing (Resizing)         (None, 78, 200, 4)        0         

=================================================================
Total params: 199,228
Trainable params: 198,988
Non-trainable params: 240
	\end{verbatim}
	\caption{Convolutional \acrshort{vae} decoder architecture.}
	\label{fig:decoder}
\end{figure*}

==> appendices/vista.tex <==
\textcolor{red}{[PLACE HOLDER] GIVE DETAILS ON VISTA ITSELF AND ON OUR CONTRIBUTIONS TO IT.}
